On the Dispersions of Three Network Information Theory Problems

We analyze the dispersions of distributed lossless source coding (the Slepian-Wolf problem), the multiple-access channel and the asymmetric broadcast channel. For the two-encoder Slepian-Wolf problem, we introduce a quantity known as the entropy dispersion matrix, which is analogous to the scalar dispersions that have gained interest recently. We prove a global dispersion result that can be expressed in terms of this entropy dispersion matrix and provides intuition on the approximate rate losses at a given blocklength and error probability. To gain better intuition about the rate at which the non-asymptotic rate region converges to the Slepian-Wolf boundary, we define and characterize two operational dispersions: the local dispersion and the weighted sum-rate dispersion. The former represents the rate of convergence to a point on the Slepian-Wolf boundary while the latter represents the fastest rate for which a weighted sum of the two rates converges to its asymptotic fundamental limit. Interestingly, when we approach either of the two corner points, the local dispersion is characterized not by a univariate Gaussian but a bivariate one as well as a subset of off-diagonal elements of the aforementioned entropy dispersion matrix. Finally, we demonstrate the versatility of our achievability proof technique by providing inner bounds for the multiple-access channel and the asymmetric broadcast channel in terms of dispersion matrices. All our proofs are unified a so-called vector rate redundancy theorem which is proved using the multidimensional Berry-Esseen theorem.

==> common_pic.tex <==
\put(0, 10){\vector(1, 0){110}}
\put(10, 0){\vector(0,1){110}}
\put(50, 30){\line(1, 0){55}}
\put(30, 50){\line(0,1){55}}
\put(50, 30){\line(-1, 1){20}}
\put(113, 10){\footnotesize $R_1$}
\put(-6, 105){\footnotesize $R_2$}
\multiput(10,50)(4,0){5}{\line(1,0){2}}
\put(-5, 50){\footnotesize $H_2$}
\put(-10, 30){\footnotesize $H_{2|1}$}
\multiput(10,30)(4,0){10}{\line(1,0){2}}
\multiput(50,10)(0,4){5}{\line(0,1){2}}
\multiput(30,10)(0,4){10}{\line(0,1){2}}
\put(50, 0){\footnotesize $H_1$}
\put(25, 0){\footnotesize $H_{1|2}$}
  \thicklines
\qbezier(40,70)(38,38)(70,40)
\put(70, 40){\line(1, 0){35}}
\put(40, 70){\line(0, 1){35}}
%\put(70, 80){\footnotesize $\scR^*_{\mathrm{SW}}(n,\epsilon)$}
\put(70, 80){\footnotesize $\scR_{\mathrm{SW}} (n,\epsilon)$}
\put(95, 22){\footnotesize $\scB^*_{\mathrm{SW}} $}
  \thinlines

==> disp_slices.tex <==
\section{Dispersion Along Slices of the $(n,\epsilon)$-Rate Regions} \label{sec:dispSlice}



==> numerical.tex <==
\begin{figure}
 \begin{center}
    \includegraphics[width=0.8\linewidth]{figs/SW_FBL_vary_n_0108}    \\
   \includegraphics[width=0.8\linewidth]{figs/SW_FBL_vary_eps_0112}    
   \end{center}
   \caption{Plots of the SW boundary  (dash-dotted black) in \eqref{eqn:sw_reg},  $(n,\epsilon)$-SW boundary (solid blue) in \eqref{eqn:ach_sw}, and the $(n,\epsilon)$-SI-ED boundary (dashed red) in \eqref{eqn:sied}  for different blocklengths  and error probabilities Notice that $\scR_{\mathrm{SW}}^*(n,\epsilon)$  and $\scR_{\mathrm{SI-ED}}^*(n,\epsilon)$  are rather  different near the equal rate and corner points when $n$ is small. Plots of $\scR_{\mathrm{SW}}^*(n,\epsilon)$  and $\scR_{\mathrm{SI-ED}}^*(n,\epsilon)$  as functions of $n$   along the  equal rate and corner point slices of $\scR_{\mathrm{SI-ED}}^*(n,\epsilon)$   are given in Figs.~\ref{fig:sum_rate} and~\ref{fig:cor_rate} respectively. These are indicated by the black $\blacktriangle$ and the green $\times$  on the plots.   The legends apply to all plots. }
   \label{fig:varyn} 
\end{figure}
 


\section{Numerical Examples}\label{sec:numeri}
In this section, we illustrate the $(n,\epsilon)$-SW region $\scR_{\mathrm{SW}}^*(n,\epsilon)$ derived in Theorem~\ref{thm:orr} and relate it to error exponent analysis~\cite{Gal76, Kos77}. We also illustrate the inner bound to the  $(n,\epsilon)$-capacity region $\scC_{\mathrm{MAC}}^*(n,\epsilon)$ for the MAC. Before we begin, we address some computational issues. In order to, for example, graph the $(n,\epsilon)$-optimal rate region for the SW problem, we find pairs of rates $(R_1, R_2)$ that lie on the boundary of $\scR_{\mathrm{SW}}^*(n,\epsilon)$. To do so, we fixed a point $R_1$ and  we performed a bisection search for $R_2$. We also  used the Matlab function \texttt{mvncdf} which returns the   cumulative probability of the multivariate normal distribution with a user-specified covariance matrix $\bV$. %This inner bound was defined in Definition~\ref{def:inner_bd_mac}.  


\subsection{Distributed Lossless Source Coding: Slepian-Wolf} \label{sec:sw_num}
In this section, we  use an example to  illustrate the $(n,\epsilon)$-SW region $\scR_{\mathrm{SW}}^*(n,\epsilon)$. We neglect the small $O(\frac{\log n}{n})$ terms in \eqref{eqn:ach_sw} and \eqref{eqn:con_sw} throughout so in fact we will plot $\tilde{\scR}_{\mathrm{SW}} (n,\epsilon)$ defined in \eqref{eqn:tildeR}. The source is taken to be  
\begin{equation}
 p_{X_1, X_2} = \begin{bmatrix} 1-3a& a\\ a & a\end{bmatrix} \label{eqn:source_sw}
\end{equation}
where $a=0.1$. This source has a positive-definite  entropy dispersion matrix $\bV(p_{X_1, X_2})$. In addition, $H(X_1)=H(X_2)=\Hb(2a)$ and $H(X_1|X_2)=H(X_2|X_1)=(1-2a)\Hb(\frac{a}{1-2a})+2a$ for this $p_{X_1,X_2}$. 



\subsubsection{Comparison to Asymptotic  SW Region and $(n,\epsilon)$-SI-ED Region}  
 In Fig.~\ref{fig:varyn}, we plot the boundary of the SW region  $\scB_{\mathrm{SW}}^*$ and the boundary of $\tilde{\scR}_{\mathrm{SW}}  (n,\epsilon)$ for different error probabilities $\epsilon$ and blocklengths $n$. We also plot the boundary of the $(n,\epsilon)$-SI-ED region  defined in \eqref{eqn:sied}. From Fig.~\ref{fig:varyn}, we see that since $\bV\succ 0$,   $\tilde{\scR}_{\mathrm{SW}}(n,\epsilon)$ has a curved boundary, reflecting the correlatedness of $X_1$ and $X_2$ and the non-degeneracy in $\bV$. We observe  from the top plots of Fig.~\ref{fig:varyn} that    $\tilde{\scR}_{\mathrm{SW}}(n,\epsilon)$  approaches the asymptotic SW boundary   $\scR_{\mathrm{SW}}^*$ as $n\to\infty$. In addition, the bottom plots of  Fig.~\ref{fig:varyn} show  that  $\tilde{\scR}_{\mathrm{SW}}(n,\epsilon) $    approaches $\scR_{\mathrm{SW}}^*$  as $\epsilon\to 1/2$.  %  as $n$ grows as demonstrated theoretically in Proposition~\ref{prop:slice}. 
 


\begin{figure}
\centering
\includegraphics[width=.8\columnwidth]{figs/SW_FBL_sum_rate_0109a}
\caption{Comparison between the $(n,\epsilon)$-SW equal rate  point and the $(n,\epsilon)$-SI-ED equal rate point as functions of $n$.   The right plot shows that the  difference in rates decays exponentially fast as predicted by \eqref{eqn:subplotb} in Proposition~\ref{prop:slices} where $\theta=\pi/4$.}
\label{fig:sum_rate}
\end{figure}

\subsubsection{Behaviour Along Certain Slices of the Regions}\label{sec:beh_slice}

There are several interesting ``slices'' of the regions shown in Fig.~\ref{fig:varyn}. Firstly, we are interested in  the equal rate  slice, which follows  along the 45$^{\circ}$ diagonal line. This is the scenario in Fig.~\ref{fig:slices}(b) with $\theta=\pi/4$. Secondly, we are also interested in   the slice passing through the origin $(0,0)$ and a {\em corner point} of  $\scR^*_{\mathrm{SI-ED}}(n,\epsilon)$,  namely $(\hatR_{1}(n,\epsilon),\hatR_{2}(n,\epsilon))$  defined    as follows:
\begin{align}
\hatR_{2}(n,\epsilon) &:=\min\{R_2 : (R_1, R_2) \in  {\scR}^*_{\mathrm{SI-ED}}(n,\epsilon) \mbox{ for some } R_1\}\nn \\*
\hatR_{1}(n,\epsilon)  &:= \min\{R_1 : (R_1,\hatR_{2}(n,\epsilon)) \in  {\scR}^*_{\mathrm{SI-ED}}(n,\epsilon) \} . \label{eqn:corner}
\end{align}
Note that the latter in \eqref{eqn:corner} is {\em not} the scenario shown in Fig.~\ref{fig:slices}(c) because we are {\em not} approaching $(H(X_1), H(X_2|X_1))$ along a straight line of a fixed slope.  These two slices are indicated by     markers ($\blacktriangle,\times$) in Fig.~\ref{fig:varyn}. The sum rates  along both slices  are  plotted as functions of $n$ in Figs.~\ref{fig:sum_rate} and~\ref{fig:cor_rate} respectively. We observe from Fig.~\ref{fig:sum_rate} that the two sum rates on the 45$^{\circ}$  equal rate line approach each other as $n$ grows. We   computed their difference and noted that it decays as $\exp(-\Theta(n))$. This is corroborated by~\eqref{eqn:subplotb}  in Proposition~\ref{prop:slices} where the difference is denoted by the exponentially decaying term $\tau_n$. This term is dominated by the $O(\frac{\log n}{n})$ residual term in Theorem~\ref{thm:orr}.    We   conclude, as we did theoretically in Section~\ref{sec:dispSlice}, that when $n$ is sufficiently large (say $n \ge 10^3$ as seen in Fig.~\ref{fig:sum_rate}), there is essentially no difference in  performing SW coding versus cooperative encoding (SI-ED) if we wish to optimize (minimize) the sum rate. The SW and SI-ED dispersions are the same and are equal to $[\bV]_{3,3}$. 

\begin{figure}
\centering
\includegraphics[width=.8\columnwidth]{figs/SW_FBL_diag_rate_0107a}
\caption{Comparison between  the $(n,\epsilon)$-SW and  $(n,\epsilon)$-SI-ED corner rates as well as  their difference  on a log-log plot. See \eqref{eqn:corner} for definitions.  In contrast to Fig.~\ref{fig:sum_rate}, note that the horizontal axis is  $\log_{10}(n)$, where $n$ is the blocklength.  The difference decays at a rate of $\Theta(n^{-1/2})$ so the dispersions of  SW   and  SI-ED  coding  along this corner rate slice are different.    }
\label{fig:cor_rate}
\end{figure} 


On the other hand, from Fig.~\ref{fig:cor_rate}, we see that the corresponding difference in corner points decays at a much slower rate of   $\mu n^{-1/2}$ for some constant  $\mu >0$. Thus,  the corner rate {\em dispersions are different} and consequently, if we wish to operate in the neighbourhood of a  corner point, SW coding  {\em loses second-order coding rate} relative to the cooperative  scenario. Intuitively, this is due to the fact that the effective dispersion approaching $(H(X_1), H(X_2|X_1))$ is a complicated function of   the conditional dispersion $[\bV]_{2,2}$, the joint dispersion $[\bV]_{3,3}$ and their correlation coefficient $\rho_{2,3}$. We discuss this in greater detail next.  % This observation is corroborated by  our theoretical result  in Proposition~\ref{prop:slice}. See Eq.~\eqref{eqn:prop_implicit}. %{\bf TODO: It would   be desirable to use Theorem~\ref{thm:orr} to analytically compute the exact dispersion at this corner point (and any other point) but this appears to be   difficult because $\scS(\bV,\epsilon)$ does not admit a closed-form expression because it  is the analogue of the cumulative distribution  function of the multivariate Gaussian $\calN(\bzero,\bV)$. }


\begin{figure}
\centering
\includegraphics[width = .55\columnwidth]{figs/angle_0117}
\caption{Plot of  $\log_{10}(F(\theta,\epsilon))$  against $\theta \in (0,3\pi/4)$ for different $\epsilon$'s. This plot  shows the ``effective dispersion'' (or second-order coding rate) as we approach the corner point $(H(X_1) , H(X_2|X_1))$ from various angles.  See Fig.~\ref{fig:slices}(c) and the definition of $F(\theta,\epsilon)$ in \eqref{eqn:R1ne} and \eqref{eqn:R2ne}. } 
\label{fig:angle}
\end{figure}
\subsubsection{Approaching a Corner Point at an Angle $\theta$}\label{sec:theta}
To better understand how the dispersion (or second-order coding rate) varies as a function of the angle of approach to a corner point, let us consider the setup in  Fig.~\ref{fig:slices}(c) and the definitions of  $R_{1 }(n,\epsilon)$ and $R_2(n,\epsilon)$ in \eqref{eqn:R1ne} and \eqref{eqn:R2ne} respectively. Recall that this rate pair $(R_{1 }(n,\epsilon),R_2(n,\epsilon))$ lies on the boundary of $\tilde{\scR}_{\mathrm{SW}}(n,\epsilon)$ and is parametrized by $F$, a dispersion-like parameter.  For the  source  defined in \eqref{eqn:source_sw}, we  solve for $F$ in \eqref{eqn:subplotc}. Hence, we are approaching the corner point $(H(X_1), H(X_2|X_1))$ at an angle $\theta$. Note that $F$ is in general a function of $\theta$ and $\epsilon$ so we write $F=F(\theta,\epsilon)$.\footnote{In fact, $F$ is also a function of $n$ as can be seen in Proposition~\ref{prop:slices}. However, it has an exponentially small dependence on $n$. In Fig.~\ref{fig:angle}, we neglect this exponentially small term when computing $F(\theta,\epsilon)$. }  In   Fig.~\ref{fig:angle},  we plot $\log_{10}(F(\theta,\epsilon))$   as a function  of $\theta \in (0, 3\pi/4)$  for different $\epsilon$'s.  It can be seen that as $\theta\to 0$, the second-order coding rate $F(\theta,\epsilon)$ increases. This agrees with intuition because when $\theta$ is small,  we are approaching the corner point $(H(X_1),H(X_2|X_1))$  almost parallel to the horizontal boundary of $\tilde{\scR}_{\mathrm{SW}}(n,\epsilon)$.  When $\theta$ is close to $3\pi/4$, similarly,  we are almost parallel  to the sum rate boundary. In either of these two cases, we are very close to the boundary of the $(n,\epsilon)$-rate region.    On the other hand, when $\theta$ is moderate (say $\theta\approx 3\pi/8$), the rate pair is  further into the interior of  $\tilde{\scR}_{\mathrm{SW}}(n,\epsilon)$, hence the effective dispersion is smaller. The  constant $3\pi/8$ is in fact not arbitrary because  the angle  between the horizontal boundary and the sum rate boundary of $\tilde{\scR}_{\mathrm{SW}}(n,\epsilon)$ is exactly $3\pi/4$.  Hence $3\pi/8$ is  the half-angle, which means that the rate pair is furthest away from either boundary.  However, the smallest dispersion does not occur at exactly $\theta= 3\pi/8$ because of some asymmetry between the entropy densities $-\log p_{X_2|X_1} (X_2|X_1)$ and $-\log p_{X_1, X_2}(X_1, X_2)$. One would also expect $F(\theta,\epsilon)$ to be  independent of  $\epsilon$ [cf.~\eqref{eqn:subplota}--\eqref{eqn:subplotb}]. However,  Fig.~\ref{fig:angle} shows that this is {\em not} the case. We conclude that the rate of convergence toward a corner point is $O(\frac{1}{\sqrt{n}})$ but the coefficient is a complicated function of $\theta$, $\epsilon$ and the model parameters in  the $2\times 2$ submatrix $[\bV]_{2:3,2:3}$.


\subsubsection{Comparison to Error Exponent Analysis}  \label{sec:comp_err} In this section, we estimate the  required blocklengths to attain an error probability $\epsilon$ using dispersion      analysis  and error exponent   analysis and we compare these estimates. Before doing so, we remind the reader of the error exponent setup and existing results. A rate pair $(R_1, R_2)$ in the (interior of the) SW region is fixed. One then asks how rapidly the error probability in~\eqref{eqn:perr_sw} decays as a function of $n$. We attempt to find  the {\em error exponent} (or {\em reliability function}) $E(R_1, R_2 )$ defined as 
\begin{equation}\label{eqn:err_exp}
E(R_1, R_2 ) :=  \limsup_{n\to\infty}    \,\, - \, \frac{1}{n}\log  \Pen  , %\doteq 2^{-n E(R_1, R_2 )}, 
\end{equation}
where here, $\Pen$ is the smallest possible error probability of length-$n$ SW block codes  with  compression rates $R_1$ and  $R_2$.  Gallager~\cite{Gal76} derived  a lower bound to  the error exponent  under maximum-likelihood decoding (MLD) for lossless source coding of $X_1$ with decoder  side information $X_2$. This was followed up by Koshelev~\cite{Kos77} who derived    a lower bound to  the error exponent  for the two-encoder SW problem (which is our setup in Section~\ref{sec:sw}). In particular, Koshelev~\cite{Kos77}  showed that the error probability  under MLD can be bounded from above as
\begin{align} 
\Pen \le 3 \exp_2 \Bigg\{    -n \max_{\rho  \in [0,1]} \min \Big[  E_{1|2}(R_1,  \rho) , 
  E_{2|1}( R_2, \rho),    E_{1,2}(R_1, R_2, \rho) \Big]   \Bigg\} \label{eqn:sw_exp}
\end{align}
where  $\exp_2(t):=2^{t}$ and the constituent exponents are defined as
\begin{align}
E_{1|2}(R_1, \rho)&:= \rho R_1 -\log \sum_{x_2} \left[ \sum_{ x_1} p_{X_1, X_2}(x_1,x_2)^{\frac{1}{1+\rho}}\right]^{1+\rho} \label{eqn:gal1} \\ 
E_{1,2}(R_1,R_2 ,\rho)&:=\rho (R_1 +R_2) -\log\left[ \sum_{x_1, x_2} p_{X_1, X_2}(x_1,x_2)^{\frac{1}{1+\rho}}\right]^{1+\rho}\label{eqn:gal2}  .
\end{align}
The exponent $E_{2|1}( R_2,\rho)$ is similar to $E_{1|2}(R_1, \rho)$ with $1$ replaced by $2$ and vice versa. Thus, the error exponent in~\eqref{eqn:err_exp} can be lower bounded as
\begin{equation}
 E(R_1, R_2 )\ge \underline{E}(R_1,R_2):= \max_{\rho\in [0,1]} \min \big[  E_{1|2}(R_1,  \rho) ,  E_{2|1}( R_2, \rho),    E_{1,2}(R_1, R_2, \rho) \big] . \label{eqn:lower_ee}
\end{equation}
%We note that if $\calX_1=\calX_2=\calX$ and $p_{X_1|X_2}(a|b)=p_{X_2|X_1}(a|b)$ for all $a,b\in\calX$, then $E_{2|1}( R, \rho)=E_{1|2}( R, \rho)$. This is indeed the case for the source in \eqref{eqn:source_sw}.  For this class of sources, the constant $3$ in \eqref{eqn:sw_exp} can be improved to $2$ as noted in~\cite[Sec.~3]{Kos77}. 
The following facts can be readily verified~\cite{Gal76, altug10} and are indeed well-known:
\begin{align}
\frac{\partial}{\partial\rho} E_{1|2}(R_1, \rho) \Big|_{\rho=0}&=R_1-H(X_1|X_2)  \label{eqn:first_der} \\
\frac{\partial^2}{\partial\rho^2} E_{1|2}(R_1, \rho) \Big|_{\rho=0}&=\var[-\log p_{X_1|X_2}(X_1|X_2)].  \label{eqn:sec_der}
\end{align}
Similar relations  hold  for the derivatives of $E_{2|1}(R_2, \rho) $ and  $E_{1,2}(R_1,R_2 ,\rho)$.   Eq.~\eqref{eqn:first_der}, together with the analogous results for $E_{2|1}(R_2, \rho) $ and  $E_{1,2}(R_1,R_2 ,\rho)$, implies that if $(R_1, R_2)$ belongs to the interior of $\scR_{\mathrm{SW}}^*$, the lower bound $\underline{E}(R_1,R_2)$ is positive so $\Pen$ decays exponentially fast. Eq.~\eqref{eqn:sec_der} shows that the second derivative of the exponent with respect to the tilting parameter $\rho$   evaluated at $\rho=0$  is precisely the (conditional)  dispersion.   This relation has found several applications in moderate deviations analysis for   information-theoretic  problems~\cite{altug10,  Tan12,  Sason11}. 


As is also well-known, the types-based characterization    by  Csisz\'{a}r and   K\"{o}rner~\cite{CK80} (see also \cite[Probs.\ 3.1.5-6]{Csi97}) coincides   with the Gallager-style    exponents in~\eqref{eqn:sw_exp}--\eqref{eqn:lower_ee}, i.e., the exponents are the same. See \cite[Prob.\ 1.2.13]{Csi97}. Even though Csisz\'{a}r-K\"{o}rner-style exponents are more intuitive, they are less amenable to numerical evaluation  because they involve  optimizing over joint distributions on $\calX_1\times\calX_2$ rather than a single scalar tilting parameter $\rho \in [0,1]$. Thus, we choose to compare our bounds to Gallager-style  error exponents.  Upper bounds on the error exponent for SW coding are provided in~\cite[Prob.\ 3.1.7]{Csi97}. It is also known that they  match the lower bound $\underline{E}(R_1,R_2)$ in~\eqref{eqn:lower_ee} when $(R_1, R_2)$ is within but close to the boundary of the achievable region~\cite[Prob.\ 3.1.7]{Csi97}. Thus for low rates, \eqref{eqn:lower_ee} is in fact an equality.  This is likened to channel coding where the sphere-packing and random coding exponents coincide above the critical rate  \cite[Sec.\ 2.5]{Csi97}. This does not come as a surprise because of the duality between Slepian-Wolf coding and channel coding \cite[Sec.~3.2]{Csi97}. 


\begin{figure}
\centering
\includegraphics[width=.8\columnwidth]{figs/cpre_bl_0113b}
\caption{Comparisons of the required blocklengths estimated by dispersion and error exponent analyses. The vertical axis is $\log_{10}(n)$, where $n$ is the blocklength.  See  further  descriptions in \eqref{eqn:disp_anal}   and~\eqref{eqn:ee_anal}. }
\label{fig:com_bl}
\end{figure}


We study estimates of the required blocklength  $n$ in the following way: We parametrize $(R_1, R_2)$   as follows: $R_1(\eta) := (1+\eta)H(X_1|X_2), R_2(\eta) := (1+\eta)H(X_2|X_1)$ for some positive number $\eta$. We ensured that $\eta$ is sufficiently large so that $R_1(\eta)+R_2(\eta)>H(X_1, X_2)$ and hence the rate pair $(R_1(\eta), R_2(\eta)) \in\scR_{\mathrm{SW}}^*$. With this parametrization,  as   the {\em deviation from the SW boundary} $\eta$ increases, the rate pair moves further into the interior of the    SW region in~\eqref{eqn:sw_reg}. We can then use two methods to estimate the critical $n$ required to achieve a target error probability $\epsilon$. The first is {\em dispersion analysis} --- we  solve for the $n$ in the bounds we derived in Theorem~\ref{thm:orr}, i.e., the least integer $n_{\mathrm{D}}$ satisfying
\begin{equation}
\rvP\big[\bZ \le \sqrt{n_{\mathrm{D}}} (\bR - \bH ) \big] \ge 1-\epsilon ,  \label{eqn:disp_anal}
\end{equation}
where $\bZ\sim\calN(\bzero,\bV)$ and $\bV$ is the   dispersion   of $p_{X_1, X_2}$. The second method is {\em error exponent analysis} --- for the  rate pair $(R_1, R_2)$, we solve for the lower bound to the  error exponent  $\underline{E} (R_1, R_2)$ in \eqref{eqn:lower_ee} and invert the relationship in~\eqref{eqn:sw_exp} to obtain  the estimate
\begin{equation}
n_{\mathrm{E}} = \left\lceil\frac{1}{ \underline{E} (R_1, R_2)}\log \left(\frac{3}{\epsilon}\right) \right\rceil. \label{eqn:ee_anal}
\end{equation}
Plots of $n_{\mathrm{D}}$ and $n_{\mathrm{E}}$ as  functions of $\eta$ and $\epsilon$ are shown in Fig.~\ref{fig:com_bl} for the source in \eqref{eqn:source_sw}. Firstly, we observe that $n$ decreases as $\eta$ increases, which agrees with our intuition that smaller blocklengths are required if the compression rates are   large. Both dispersion and error exponent analysis exhibit the same trend. Secondly, we  observe that   dispersion analysis generally  predicts a smaller blocklength compared to Gallager-style error exponent analysis. As an example, when $\eta=0.1$ and $\epsilon = 10^{-3}$,  $n_{\mathrm{D}}\approx 9.9\times 10^{3}$ while $n_{\mathrm{E}}\approx 1.6\times 10^{4}$. Thus, the required blocklength estimated by dispersion analysis is about 39\% less than error exponent analysis for this setting.  Dispersion analysis is, in a sense,  {\em more delicate}  (or \emph{finer}) than that of error exponents~\cite{Gal76, Kos77, CK80}. The difference, however, is less pronounced as the rates increase. In other words,  the estimates of $n$ become closer (on a linear  not logarithmic scale) as the rates are further into the SW region.




\subsection{Multiple-Access Channel}


\begin{figure}
 \begin{center}
    \includegraphics[width=0.8\linewidth]{figs/MAC_FBL_0108}    \\
   \includegraphics[width=0.8\linewidth]{figs/MAC_FBL_vary_eps_0115}    
   \end{center}
   \caption{Plots of the MAC boundary in \eqref{eqn:mac_reg} and the $(n,\epsilon)$-inner bound in~\eqref{eqn:ach_mac} for different blocklengths and error probabilities.  Here $p_{X_1} =\Ber(0.1)$ and $p_{X_2}= \Ber(0.9)$ are fixed input distributions. The time-sharing variable $Q=\emptyset$. The legends apply to all plots.}
   \label{fig:mac} 
\end{figure}

In this section, we illustrate the differences between the asymptotic MAC region and the finite blocklength MAC region $\scC^*_{\mathrm{MAC}}(n, \epsilon)$. In fact, we only graph the inner bound in Definition~\ref{def:inner_bd_mac} as we do not yet have an outer bound.  We fix a channel with binary inputs and binary outputs:
\begin{equation}
W(\, \, : \, |x_1, x_2 ) = \begin{cases} [\bar{b}\,\,\,\, b  ] & \text{if $x_1\oplus x_2 = 0$,}
\\
[b\,\,\,\,\bar{b}  ] & \text{if $x_1\oplus x_2 = 1$,}
\end{cases}
%W(\, : \, |x_1, x_2 ) =\left\{ \begin{array}{cc} [1-a\,\, a] & x_1\oplus x_2 = 0 \\ [1-b\,\, b] & x_1 \oplus x_2 = 1 \end{array} \right.
\end{equation}
where $b=0.1$ and $\bar{b} :=1-b$.  We also fix input distributions $p_{X_1} =\Ber(b)$ and $p_{X_2}= \Ber(\bar{b})$. The time-sharing variable $Q=\emptyset$. This channel and input distributions result in a positive-definite information dispersion matrix $\bV$ defined in~\eqref{eqn:macv}.   These settings also  ensure that we have symmetry in the sense that  $I(X_1;Y)=I(X_2;Y)$ and $I(X_1;Y|X_2)=I(X_2;Y|X_2)$.  In Fig.~\ref{fig:mac}, we graph the MAC region in~\eqref{eqn:mac_reg} which is well known to be  a pentagon.  We also  plot the inner bound    in~\eqref{eqn:ach_mac} for the chosen $p_{X_1} , p_{X_2}$ for  different  values of the blocklength $n$ and error probability $\epsilon$.     Note again that the $O(\frac{\log n}{n})$ term is neglected because we are   primarily interested in this paper with  first- and second-order coding rates. In addition, we   plot the $(n,\epsilon)$-SI-ED boundary. This is the analogue of~\eqref{eqn:sied} for the SW case.  More precisely, the vertical (resp.\ horizontal) boundary represents the $(n,\epsilon)$-capacity  of a DMC when $X_2$ (resp.\ $X_1$) is   available as side information at the decoder together with channel output $Y$. The sloping (dotted-red) line $R_1+R_2=I(X_1,X_2;Y)-\sqrt{ [\bV]_{3,3}/n}\,\rmQ^{-1}(\epsilon)$ represents the $(n,\epsilon)$-sum rate constraint of the DM-MAC. Operationally, it represents the $(n,\epsilon)$-capacity of the ``cooperative MAC'' but with independent messages. These are three crude outer bounds that turn out to be  insufficient for the DM-MAC. 

We see that as in the SW case, the inner bound to the $(n,\epsilon)$-capacity region is, as expected, strictly contained in the asymptotic MAC region. Furthermore, it has a curved boundary in general and the larger the blocklength $n$, the closer the inner bound is to the asymptotic region.   The different behaviours of the $(n,\epsilon)$-region  along the equal rate line and the line that passes through a corner point [cf.~\eqref{eqn:corner}] are qualitatively similar to the SW case described in Section~\ref{sec:sw_num} so we will omit the  corresponding plots. We do note that, in analogy to Proposition~\ref{prop:slices} for the SW case, at  any rate $R_1<I(X;Y_1)$, the difference between the two different $R_2$'s (asymptotic and finite blocklength) is  essentially    $\sqrt{[ \bV]_{2,2}/n} \, \rmQ^{-1}(\epsilon)$ where    $[\bV]_{2,2} = \var(\log [  W(Y|X_1,X_2)/p_{Y|X_1}(Y|X_1) ])$ is the conditional  channel dispersion. Finally, the corner points exhibit more complex behaviours; the effective dispersion depends on the angle of approach and the correlation between the marginal and joint information densities.


